Constraining models for the origin of ultra-high-energy cosmic rays with a novel combined analysis of arrival directions, spectrum, and composition data measured at the Pierre Auger Observatory

The combined fit of the measured energy spectrum and shower maximum depth distributions of ultra-high-energy cosmic rays is known to constrain the parameters of astrophysical models with homogeneous source distributions. Studies of the distribution of the cosmic-ray arrival directions show a better agreement with models in which a fraction of the flux is non-isotropic and associated with the nearby radio galaxy Centaurus A or with catalogs such as that of starburst galaxies. Here, we present a novel combination of both analyses by a simultaneous fit of arrival directions, energy spectrum, and composition data measured at the Pierre Auger Observatory. We find that a model containing a flux contribution from the starburst galaxy catalog of around 20% at 40 EeV with a magnetic field blurring of around $20^\circ$ for a rigidity of 10 EV provides a fair simultaneous description of all three observables. The starburst galaxy model is favored with a significance of $4.5\sigma$ (considering experimental systematic effects) compared to a reference model with only homogeneously distributed background sources. By investigating a scenario with Centaurus A as a single source in combination with the homogeneous background, we confirm that this region of the sky provides the dominant contribution to the observed anisotropy signal. Models containing a catalog of jetted active galactic nuclei whose flux scales with the $\gamma$-ray emission are, however, disfavored as they cannot adequately describe the measured arrival directions.

==> Makefile <==
# Makefile for building latex documents (c) Darko Veberic
# $Id: Makefile 13376 2021-08-04 17:24:17Z darko $

USEPDFLATEX := 1
USEBIBTEX := 0

TEXFILES := $(shell grep -le '^\s*\\document\(class\|style\)' *.tex)
TARGETS := $(basename $(TEXFILES))
DEPENDENCIES := $(wildcard *.sty *.bib figs/*) $(filter-out $(TEXFILES), $(wildcard *.tex))

##########################################################
SHELL := /bin/bash
PDFS := $(addsuffix .pdf, $(TARGETS))

ifeq (, $(shell which latexmk))
  LATEX := $(if $(filter 1, $(USEPDFLATEX)), pdflatex, latex)
  # 30=black 31=red 32=green 33=yellow 34=blue 35=magenta 36=cyan 37=white 0=cancel
  COLORIZE := awk 'BEGIN{ec="\033[31;1m";wc="\033[34;1m";cc="\033[0m"}/Rerun /||/rerunfilecheck[^.]/{e=e$$0"\n";print ec""$$0""cc;next}/^LaTeX Warning:/||/natbib Warning:/{w=w$$0"\n";print wc""$$0""cc;next}{print}END{if(w||e)print "\n"ec"Warning/error summary:"cc"\n"wc""w""cc;if(e){print ec""e""cc;exit 1}}'
  define basic_latex_rule
    for i in 1 2 3 ; do $(LATEX) $< | $(COLORIZE) && break ; done
  endef
  ifeq ($(USEBIBTEX), 1)
    define latex_rule
      $(LATEX) $< ; bibtex $*
      $(call basic_latex_rule)
    endef
  else
    define latex_rule
      $(call basic_latex_rule)
    endef
  endif
else
  define latex_rule
    latexmk $(if $(filter 1, $(USEPDFLATEX)), -pdf, ) $<
  endef
endif

.PHONY: all clean

all: $(PDFS)

# dependencies
$(PDFS): $(DEPENDENCIES)

clean:
	- $(RM) *{.tex~,.dvi,.log,.aux,.toc,.nav,.out,.snm,.bbl,.blg,.spl,.lof,Notes.bib,.maf,.fff,.lot,.ttt,.bcf,.run.xml,.fdb_latexmk,.fls,.synctex.gz}
	- for f in $(TARGETS) ; do $(RM) $$f{.ps,.pdf} ; done

# general rules
ifeq ($(USEPDFLATEX), 1)
%.pdf: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.ps: %.pdf
	pdf2ps $<
else
%.dvi: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.pdf: %.dvi
	dvipdf $<

%.ps: %.dvi
	dvips $< -o
endif

# embed pdf fonts
%.embedded_fonts.pdf: %.pdf
	gs -dSAFER -dNOPLATFONTS -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sPAPERSIZE=a4 -dCompatibilityLevel=1.4 -dPDFSETTINGS=/printer -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sOutputFile=$@ -f $<


==> auger_authors_short.tex <==
\author[1]{The Pierre Auger Collaboration}

\affiliation[1]{Exchange with real author list \textit{jcappub\_authorlist} when ready}

==> img/jcappub_authorlist.tex <==
% created on 2023-04-05
\author[13]{A.~Abdul Halim,}
\author[72]{P.~Abreu,}
\author[54,52]{M.~Aglietta,}
\author[1]{I.~Allekotte,}
\author[70]{K.~Almeida Cheminant,}
\author[7,12]{A.~Almela,}
\author[45,46]{R.~Aloisio,}
\author[79]{J.~Alvarez-Mu\~niz,}
\author[79]{J.~Ammerman Yebra,}
\author[54,52]{G.A.~Anastasi,}
\author[86]{L.~Anchordoqui,}
\author[7]{B.~Andrada,}
\author[72]{S.~Andringa,}
\author[50]{C.~Aramo,}
\author[42]{P.R.~Ara\'ujo Ferreira,}
\author[63,52]{E.~Arnone,}
\author[67]{J.~C.~Arteaga Vel\'azquez,}
\author[7]{H.~Asorey,}
\author[72]{P.~Assis,}
\author[11]{G.~Avila,}
\author[57,46]{E.~Avocone,}
\author[75]{A.M.~Badescu,}
\author[32]{A.~Bakalova,}
\author[73]{A.~Balaceanu,}
\author[45,46]{F.~Barbato,}
\author[85]{A.~Bartz Mocellin,}
\author[13,69]{J.A.~Bellido,}
\author[36]{C.~Berat,}
\author[63,52]{M.E.~Bertaina,}
\author[70]{G.~Bhatta,}
\author[63,52]{M.~Bianciotto,}
\author[h]{P.L.~Biermann,}
\author[5]{V.~Binet,}
\author[39,7]{K.~Bismark,}
\author[80,81]{T.~Bister,}
\author[37]{J.~Biteau,}
\author[32]{J.~Blazek,}
\author[36]{C.~Bleve,}
\author[41]{J.~Bl\"umer,}
\author[32]{M.~Boh\'a\v{c}ov\'a,}
\author[57,46]{D.~Boncioli,}
\author[8,26]{C.~Bonifazi,}
\author[21]{L.~Bonneau Arbeletche,}
\author[70]{N.~Borodai,}
\author[j]{J.~Brack,}
\author[7]{P.G.~Brichetto Orchera,}
\author[42]{F.L.~Briechle,}
\author[78]{A.~Bueno,}
\author[15]{S.~Buitink,}
\author[47,61]{M.~Buscemi,}
\author[39,7]{M.~B\"usken,}
\author[80,81]{A.~Bwembya,}
\author[66]{K.S.~Caballero-Mora,}
\author[59,49]{L.~Caccianiga,}
\author[38]{I.~Caracas,}
\author[58,47]{R.~Caruso,}
\author[54,52]{A.~Castellina,}
\author[18]{F.~Catalani,}
\author[48]{G.~Cataldi,}
\author[79]{L.~Cazon,}
\author[10]{M.~Cerda,}
\author[21]{J.A.~Chinellato,}
\author[32]{J.~Chudoba,}
\author[33]{L.~Chytka,}
\author[13]{R.W.~Clay,}
\author[6]{A.C.~Cobos Cerutti,}
\author[60,50]{R.~Colalillo,}
\author[90]{A.~Coleman,}
\author[48]{M.R.~Coluccia,}
\author[72]{R.~Concei\c{c}\~ao,}
\author[37]{A.~Condorelli,}
\author[49,55]{G.~Consolati,}
\author[56,48]{M.~Conte,}
\author[41]{F.~Convenga,}
\author[28]{D.~Correia dos Santos,}
\author[72]{P.J.~Costa,}
\author[84]{C.E.~Covault,}
\author[44]{M.~Cristinziani,}
\author[3]{C.S.~Cruz Sanchez,}
\author[4,2]{S.~Dasso,}
\author[41]{K.~Daumiller,}
\author[13]{B.R.~Dawson,}
\author[28]{R.M.~de Almeida,}
\author[7,41]{J.~de Jes\'us,}
\author[80,81]{S.J.~de Jong,}
\author[26,27]{J.R.T.~de Mello Neto,}
\author[45,46]{I.~De Mitri,}
\author[17]{J.~de Oliveira,}
\author[21]{D.~de Oliveira Franco,}
\author[56,48]{F.~de Palma,}
\author[19]{V.~de Souza,}
\author[56,48]{E.~De Vito,}
\author[58,47]{A.~Del Popolo,}
\author[34]{O.~Deligny,}
\author[41,7]{L.~Deval,}
\author[52]{A.~di Matteo,}
\author[73]{M.~Dobre,}
\author[21]{C.~Dobrigkeit,}
\author[68]{J.C.~D'Olivo,}
\author[72]{L.M.~Domingues Mendes,}
\author[]{J.C.~dos Anjos,}
\author[25]{R.C.~dos Anjos,}
\author[32]{J.~Ebr,}
\author[80,81]{M.~Emam,}
\author[39,41]{R.~Engel,}
\author[56,48]{I.~Epicoco,}
\author[42]{M.~Erdmann,}
\author[7,12]{A.~Etchegoyen,}
\author[45,46]{C.~Evoli,}
\author[80,82,81]{H.~Falcke,}
\author[89]{J.~Farmer,}
\author[88]{G.~Farrar,}
\author[21]{A.C.~Fauth,}
\author[e]{N.~Fazzini,}
\author[40]{F.~Feldbusch,}
\author[41,d]{F.~Fenu,}
\author[72]{A.~Fernandes,}
\author[87]{B.~Fick,}
\author[7]{J.M.~Figueira,}
\author[77,76]{A.~Filip\v{c}i\v{c},}
\author[41]{T.~Fitoussi,}
\author[90]{B.~Flaggs,}
\author[80]{T.~Fodran,}
\author[89,f]{T.~Fujii,}
\author[7,12]{A.~Fuster,}
\author[80]{C.~Galea,}
\author[59,49]{C.~Galelli,}
\author[6]{B.~Garc\'\i{}a,}
\author[38]{C.~Gaudu,}
\author[40]{H.~Gemmeke,}
\author[7,41]{F.~Gesualdi,}
\author[73]{A.~Gherghel-Lascu,}
\author[34]{P.L.~Ghia,}
\author[48]{U.~Giaccari,}
\author[49]{M.~Giammarchi,}
\author[42,g]{J.~Glombitza,}
\author[10]{F.~Gobbi,}
\author[7]{F.~Gollan,}
\author[1]{G.~Golup,}
\author[1]{M.~G\'omez Berisso,}
\author[11]{P.F.~G\'omez Vitale,}
\author[11]{J.P.~Gongora,}
\author[1]{J.M.~Gonz\'alez,}
\author[7]{N.~Gonz\'alez,}
\author[1]{I.~Goos,}
\author[70]{D.~G\'ora,}
\author[54,52]{A.~Gorgi,}
\author[79]{M.~Gottowik,}
\author[13]{T.D.~Grubb,}
\author[60,50]{F.~Guarino,}
\author[22]{G.P.~Guedes,}
\author[44]{E.~Guido,}
\author[39]{S.~Hahn,}
\author[32]{P.~Hamal,}
\author[7]{M.R.~Hampel,}
\author[3]{P.~Hansen,}
\author[1]{D.~Harari,}
\author[13]{V.M.~Harvey,}
\author[41]{A.~Haungs,}
\author[42]{T.~Hebbeker,}
\author[e]{C.~Hojvat,}
\author[80,81]{J.R.~H\"orandel,}
\author[33]{P.~Horvath,}
\author[33]{M.~Hrabovsk\'y,}
\author[41,15]{T.~Huege,}
\author[58,47]{A.~Insolia,}
\author[74]{P.G.~Isar,}
\author[32]{P.~Janecek,}
\author[85]{J.A.~Johnsen,}
\author[32]{J.~Jurysek,}
\author[38]{A.~K\"a\"ap\"a,}
\author[38]{K.H.~Kampert,}
\author[41]{B.~Keilhauer,}
\author[80]{A.~Khakurdikar,}
\author[7,41]{V.V.~Kizakke Covilakam,}
\author[41]{H.O.~Klages,}
\author[40]{M.~Kleifges,}
\author[39]{F.~Knapp,}
\author[40]{N.~Kunka,}
\author[16]{B.L.~Lago,}
\author[42]{N.~Langner,}
\author[24]{M.A.~Leigui de Oliveira,}
\author[79]{Y Lema-Capeans,}
\author[39]{V.~Lenok,}
\author[35]{A.~Letessier-Selvon,}
\author[34]{I.~Lhenry-Yvon,}
\author[58,47]{D.~Lo Presti,}
\author[72]{L.~Lopes,}
\author[64]{R.~L\'opez,}
\author[91]{L.~Lu,}
\author[39]{Q.~Luce,}
\author[76]{J.P.~Lundquist,}
\author[21]{A.~Machado Payeras,}
\author[32]{M.~Majercakova,}
\author[32]{D.~Mandat,}
\author[13]{B.C.~Manning,}
\author[e]{P.~Mantsch,}
\author[34]{S.~Marafico,}
\author[59,49]{F.M.~Mariani,}
\author[3]{A.G.~Mariazzi,}
\author[14]{I.C.~Mari\c{s},}
\author[61,47]{G.~Marsella,}
\author[56,48]{D.~Martello,}
\author[41,7]{S.~Martinelli,}
\author[64]{O.~Mart\'\i{}nez Bravo,}
\author[79]{M.A.~Martins,}
\author[57,46]{M.~Mastrodicasa,}
\author[41]{H.J.~Mathes,}
\author[a]{J.~Matthews,}
\author[62,51]{G.~Matthiae,}
\author[85,38]{E.~Mayotte,}
\author[85]{S.~Mayotte,}
\author[e]{P.O.~Mazur,}
\author[68]{G.~Medina-Tanco,}
\author[38]{J.~Meinert,}
\author[7]{D.~Melo,}
\author[40]{A.~Menshikov,}
\author[41]{C.~Merx,}
\author[33]{S.~Michal,}
\author[5]{M.I.~Micheletti,}
\author[59,49]{L.~Miramonti,}
\author[1]{S.~Mollerach,}
\author[36]{F.~Montanet,}
\author[38]{L.~Morejon,}
\author[54,52]{C.~Morello,}
\author[32]{A.L.~M\"uller,}
\author[80,81]{K.~Mulrey,}
\author[52]{R.~Mussa,}
\author[88]{M.~Muzio,}
\author[38]{W.M.~Namasaka,}
\author[38]{A.~Nasr-Esfahani,}
\author[68]{L.~Nellen,}
\author[9]{G.~Nicora,}
\author[73]{M.~Niculescu-Oglinzanu,}
\author[44]{M.~Niechciol,}
\author[87]{D.~Nitz,}
\author[31]{D.~Nosek,}
\author[31]{V.~Novotny,}
\author[33]{L.~No\v{z}ka,}
\author[56,48]{A Nucita,}
\author[30]{L.A.~N\'u\~nez,}
\author[19]{C.~Oliveira,}
\author[32]{M.~Palatka,}
\author[9]{J.~Pallotta,}
\author[79]{G.~Parente,}
\author[64]{A.~Parra,}
\author[38]{J.~Pawlowsky,}
\author[32]{M.~Pech,}
\author[70]{J.~P\c{e}kala,}
\author[65]{R.~Pelayo,}
\author[23]{L.A.S.~Pereira,}
\author[39,7]{E.E.~Pereira Martins,}
\author[20]{J.~Perez Armand,}
\author[7,41]{C.~P\'erez Bertolli,}
\author[56,48]{L.~Perrone,}
\author[45,46]{S.~Petrera,}
\author[57,46]{C.~Petrucci,}
\author[41]{T.~Pierog,}
\author[72]{M.~Pimenta,}
\author[7]{M.~Platino,}
\author[80]{B.~Pont,}
\author[81,80]{M.~Pothast,}
\author[61,47]{M.~Pourmohammad Shahvar,}
\author[89]{P.~Privitera,}
\author[32]{M.~Prouza,}
\author[87]{A.~Puyleart,}
\author[38]{S.~Querchfeld,}
\author[38]{J.~Rautenberg,}
\author[7]{D.~Ravignani,}
\author[39]{M.~Reininghaus,}
\author[32]{J.~Ridky,}
\author[79]{F.~Riehn,}
\author[44]{M.~Risse,}
\author[57,46]{V.~Rizi,}
\author[80]{W.~Rodrigues de Carvalho,}
\author[11]{J.~Rodriguez Rojo,}
\author[10]{M.~Rojas,}
\author[7]{M.J.~Roncoroni,}
\author[43]{S.~Rossoni,}
\author[41]{M.~Roth,}
\author[4]{A.C.~Rovero,}
\author[44]{P.~Ruehl,}
\author[73]{A.~Saftoiu,}
\author[80]{M.~Saharan,}
\author[57,46]{F.~Salamida,}
\author[64]{H.~Salazar,}
\author[51]{G.~Salina,}
\author[30]{J.D.~Sanabria Gomez,}
\author[7]{F.~S\'anchez,}
\author[20]{E.M.~Santos,}
\author[32]{E.~Santos,}
\author[85]{F.~Sarazin,}
\author[72]{R.~Sarmento,}
\author[11]{R.~Sato,}
\author[91]{P.~Savina,}
\author[41]{C.M.~Sch\"afer,}
\author[56,48]{V.~Scherini,}
\author[41]{H.~Schieler,}
\author[34]{M.~Schimassek,}
\author[38]{M.~Schimp,}
\author[41]{F.~Schl\"uter,}
\author[39]{D.~Schmidt,}
\author[15,i]{O.~Scholten,}
\author[80,81]{H.~Schoorlemmer,}
\author[32]{P.~Schov\'anek,}
\author[90,41]{F.G.~Schr\"oder,}
\author[42]{J.~Schulte,}
\author[41]{T.~Schulz,}
\author[3]{S.J.~Sciutto,}
\author[7,41]{M.~Scornavacche,}
\author[53,47]{A.~Segreto,}
\author[38]{S.~Sehgal,}
\author[76]{S.U.~Shivashankara,}
\author[43]{G.~Sigl,}
\author[7]{G.~Silli,}
\author[73,b]{O.~Sima,}
\author[40]{F.~Simon,}
\author[73]{R.~Smau,}
\author[89]{R.~\v{S}m\'\i{}da,}
\author[k]{P.~Sommers,}
\author[86]{J.F.~Soriano,}
\author[10]{R.~Squartini,}
\author[32]{M.~Stadelmaier,}
\author[73]{D.~Stanca,}
\author[76]{S.~Stani\v{c},}
\author[70]{J.~Stasielak,}
\author[36]{P.~Stassi,}
\author[42]{M.~Straub,}
\author[39,7]{A.~Streich,}
\author[14]{M.~Su\'arez-Dur\'an,}
\author[37]{T.~Suomij\"arvi,}
\author[7]{A.D.~Supanitsky,}
\author[32]{Z.~Svozilikova,}
\author[71]{Z.~Szadkowski,}
\author[29]{A.~Tapia,}
\author[63,52]{C.~Taricco,}
\author[81,80]{C.~Timmermans,}
\author[41]{O.~Tkachenko,}
\author[32]{P.~Tobiska,}
\author[18]{C.J.~Todero Peixoto,}
\author[72]{B.~Tom\'e,}
\author[36]{Z.~Torr\`es,}
\author[10]{A.~Travaini,}
\author[32]{P.~Travnicek,}
\author[57,46]{C.~Trimarelli,}
\author[3]{M.~Tueros,}
\author[41]{M.~Unger,}
\author[33]{L.~Vaclavek,}
\author[33]{M.~Vacula,}
\author[68]{J.F.~Vald\'es Galicia,}
\author[60,50]{L.~Valore,}
\author[64]{E.~Varela,}
\author[30]{A.~V\'asquez-Ram\'\i{}rez,}
\author[41]{D.~Veberi\v{c},}
\author[27]{C.~Ventura,}
\author[3]{I.D.~Vergara Quispe,}
\author[51]{V.~Verzi,}
\author[32]{J.~Vicha,}
\author[83]{J.~Vink,}
\author[32]{J.~Vlastimil,}
\author[76]{S.~Vorobiov,}
\author[26]{C.~Watanabe,}
\author[c]{A.A.~Watson,}
\author[41]{A.~Weindl,}
\author[85]{L.~Wiencke,}
\author[70]{H.~Wilczy\'nski,}
\author[38]{D.~Wittkowski,}
\author[7]{B.~Wundheiler,}
\author[38]{B.~Yue,}
\author[32]{A.~Yushkov,}
\author[14]{O.~Zapparrata,}
\author[79]{E.~Zas,}
\author[76,77]{D.~Zavrtanik,}
\author[77,76]{and M.~Zavrtanik}

\affiliation[1]{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}
\affiliation[2]{Departamento de F\'\i{}sica and Departamento de Ciencias de la Atm\'osfera y los Oc\'eanos, FCEyN, Universidad de Buenos Aires and CONICET, Buenos Aires, Argentina}
\affiliation[3]{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}
\affiliation[4]{Instituto de Astronom\'\i{}a y F\'\i{}sica del Espacio (IAFE, CONICET-UBA), Buenos Aires, Argentina}
\affiliation[5]{Instituto de F\'\i{}sica de Rosario (IFIR) -- CONICET/U.N.R.\ and Facultad de Ciencias Bioqu\'\i{}micas y Farmac\'euticas U.N.R., Rosario, Argentina}
\affiliation[6]{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), and Universidad Tecnol\'ogica Nacional -- Facultad Regional Mendoza (CONICET/CNEA), Mendoza, Argentina}
\affiliation[7]{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation[8]{International Center of Advanced Studies and Instituto de Ciencias F\'\i{}sicas, ECyT-UNSAM and CONICET, Campus Miguelete -- San Mart\'\i{}n, Buenos Aires, Argentina}
\affiliation[9]{Laboratorio Atm\'osfera -- Departamento de Investigaciones en L\'aseres y sus Aplicaciones -- UNIDEF (CITEDEF-CONICET), Argentina}
\affiliation[10]{Observatorio Pierre Auger, Malarg\"ue, Argentina}
\affiliation[11]{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina}
\affiliation[12]{Universidad Tecnol\'ogica Nacional -- Facultad Regional Buenos Aires, Buenos Aires, Argentina}
\affiliation[13]{University of Adelaide, Adelaide, S.A., Australia}
\affiliation[14]{Universit\'e Libre de Bruxelles (ULB), Brussels, Belgium}
\affiliation[15]{Vrije Universiteit Brussels, Brussels, Belgium}
\affiliation[16]{Centro Federal de Educa\c{c}\~ao Tecnol\'ogica Celso Suckow da Fonseca, Petropolis, Brazil}
\affiliation[17]{Instituto Federal de Educa\c{c}\~ao, Ci\^encia e Tecnologia do Rio de Janeiro (IFRJ), Brazil}
\affiliation[18]{Universidade de S\~ao Paulo, Escola de Engenharia de Lorena, Lorena, SP, Brazil}
\affiliation[19]{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica de S\~ao Carlos, S\~ao Carlos, SP, Brazil}
\affiliation[20]{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica, S\~ao Paulo, SP, Brazil}
\affiliation[21]{Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil}
\affiliation[22]{Universidade Estadual de Feira de Santana, Feira de Santana, Brazil}
\affiliation[23]{Universidade Federal de Campina Grande, Centro de Ciencias e Tecnologia, Campina Grande, Brazil}
\affiliation[24]{Universidade Federal do ABC, Santo Andr\'e, SP, Brazil}
\affiliation[25]{Universidade Federal do Paran\'a, Setor Palotina, Palotina, Brazil}
\affiliation[26]{Universidade Federal do Rio de Janeiro, Instituto de F\'\i{}sica, Rio de Janeiro, RJ, Brazil}
\affiliation[27]{Universidade Federal do Rio de Janeiro (UFRJ), Observat\'orio do Valongo, Rio de Janeiro, RJ, Brazil}
\affiliation[28]{Universidade Federal Fluminense, EEIMVR, Volta Redonda, RJ, Brazil}
\affiliation[29]{Universidad de Medell\'\i{}n, Medell\'\i{}n, Colombia}
\affiliation[30]{Universidad Industrial de Santander, Bucaramanga, Colombia}
\affiliation[31]{Charles University, Faculty of Mathematics and Physics, Institute of Particle and Nuclear Physics, Prague, Czech Republic}
\affiliation[32]{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}
\affiliation[33]{Palacky University, Olomouc, Czech Republic}
\affiliation[34]{CNRS/IN2P3, IJCLab, Universit\'e Paris-Saclay, Orsay, France}
\affiliation[35]{Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Sorbonne Universit\'e, Universit\'e de Paris, CNRS-IN2P3, Paris, France}
\affiliation[36]{Univ.\ Grenoble Alpes, CNRS, Grenoble Institute of Engineering Univ.\ Grenoble Alpes, LPSC-IN2P3, 38000 Grenoble, France}
\affiliation[37]{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France}
\affiliation[38]{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}
\affiliation[39]{Karlsruhe Institute of Technology (KIT), Institute for Experimental Particle Physics, Karlsruhe, Germany}
\affiliation[40]{Karlsruhe Institute of Technology (KIT), Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany}
\affiliation[41]{Karlsruhe Institute of Technology (KIT), Institute for Astroparticle Physics, Karlsruhe, Germany}
\affiliation[42]{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}
\affiliation[43]{Universit\"at Hamburg, II.\ Institut f\"ur Theoretische Physik, Hamburg, Germany}
\affiliation[44]{Universit\"at Siegen, Department Physik -- Experimentelle Teilchenphysik, Siegen, Germany}
\affiliation[45]{Gran Sasso Science Institute, L'Aquila, Italy}
\affiliation[46]{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}
\affiliation[47]{INFN, Sezione di Catania, Catania, Italy}
\affiliation[48]{INFN, Sezione di Lecce, Lecce, Italy}
\affiliation[49]{INFN, Sezione di Milano, Milano, Italy}
\affiliation[50]{INFN, Sezione di Napoli, Napoli, Italy}
\affiliation[51]{INFN, Sezione di Roma ``Tor Vergata'', Roma, Italy}
\affiliation[52]{INFN, Sezione di Torino, Torino, Italy}
\affiliation[53]{Istituto di Astrofisica Spaziale e Fisica Cosmica di Palermo (INAF), Palermo, Italy}
\affiliation[54]{Osservatorio Astrofisico di Torino (INAF), Torino, Italy}
\affiliation[55]{Politecnico di Milano, Dipartimento di Scienze e Tecnologie Aerospaziali , Milano, Italy}
\affiliation[56]{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation[57]{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy}
\affiliation[58]{Universit\`a di Catania, Dipartimento di Fisica e Astronomia ``Ettore Majorana``, Catania, Italy}
\affiliation[59]{Universit\`a di Milano, Dipartimento di Fisica, Milano, Italy}
\affiliation[60]{Universit\`a di Napoli ``Federico II'', Dipartimento di Fisica ``Ettore Pancini'', Napoli, Italy}
\affiliation[61]{Universit\`a di Palermo, Dipartimento di Fisica e Chimica ''E.\ Segr\`e'', Palermo, Italy}
\affiliation[62]{Universit\`a di Roma ``Tor Vergata'', Dipartimento di Fisica, Roma, Italy}
\affiliation[63]{Universit\`a Torino, Dipartimento di Fisica, Torino, Italy}
\affiliation[64]{Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}
\affiliation[65]{Unidad Profesional Interdisciplinaria en Ingenier\'\i{}a y Tecnolog\'\i{}as Avanzadas del Instituto Polit\'ecnico Nacional (UPIITA-IPN), M\'exico, D.F., M\'exico}
\affiliation[66]{Universidad Aut\'onoma de Chiapas, Tuxtla Guti\'errez, Chiapas, M\'exico}
\affiliation[67]{Universidad Michoacana de San Nicol\'as de Hidalgo, Morelia, Michoac\'an, M\'exico}
\affiliation[68]{Universidad Nacional Aut\'onoma de M\'exico, M\'exico, D.F., M\'exico}
\affiliation[69]{Universidad Nacional de San Agustin de Arequipa, Facultad de Ciencias Naturales y Formales, Arequipa, Peru}
\affiliation[70]{Institute of Nuclear Physics PAN, Krakow, Poland}
\affiliation[71]{University of \L{}\'od\'z, Faculty of High-Energy Astrophysics,\L{}\'od\'z, Poland}
\affiliation[72]{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}
\affiliation[73]{``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania}
\affiliation[74]{Institute of Space Science, Bucharest-Magurele, Romania}
\affiliation[75]{University Politehnica of Bucharest, Bucharest, Romania}
\affiliation[76]{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}
\affiliation[77]{Experimental Particle Physics Department, J.\ Stefan Institute, Ljubljana, Slovenia}
\affiliation[78]{Universidad de Granada and C.A.F.P.E., Granada, Spain}
\affiliation[79]{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}
\affiliation[80]{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\affiliation[81]{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}
\affiliation[82]{Stichting Astronomisch Onderzoek in Nederland (ASTRON), Dwingeloo, The Netherlands}
\affiliation[83]{Universiteit van Amsterdam, Faculty of Science, Amsterdam, The Netherlands}
\affiliation[84]{Case Western Reserve University, Cleveland, OH, USA}
\affiliation[85]{Colorado School of Mines, Golden, CO, USA}
\affiliation[86]{Department of Physics and Astronomy, Lehman College, City University of New York, Bronx, NY, USA}
\affiliation[87]{Michigan Technological University, Houghton, MI, USA}
\affiliation[88]{New York University, New York, NY, USA}
\affiliation[89]{University of Chicago, Enrico Fermi Institute, Chicago, IL, USA}
\affiliation[90]{University of Delaware, Department of Physics and Astronomy, Bartol Research Institute, Newark, DE, USA}
\affiliation[91]{University of Wisconsin-Madison, Department of Physics and WIPAC, Madison, WI, USA}
\affiliation[]{-----}
\affiliation[a]{Louisiana State University, Baton Rouge, LA, USA}
\affiliation[b]{also at University of Bucharest, Physics Department, Bucharest, Romania}
\affiliation[c]{School of Physics and Astronomy, University of Leeds, Leeds, United Kingdom}
\affiliation[d]{now at Agenzia Spaziale Italiana (ASI).\ Via del Politecnico 00133, Roma, Italy}
\affiliation[e]{Fermi National Accelerator Laboratory, Fermilab, Batavia, IL, USA}
\affiliation[f]{now at Graduate School of Science, Osaka Metropolitan University, Osaka, Japan}
\affiliation[g]{now at ECAP, Erlangen, Germany}
\affiliation[h]{Max-Planck-Institut f\"ur Radioastronomie, Bonn, Germany}
\affiliation[i]{also at Kapteyn Institute, University of Groningen, Groningen, The Netherlands}
\affiliation[j]{Colorado State University, Fort Collins, CO, USA}
\affiliation[k]{Pennsylvania State University, University Park, PA, USA}

